Bridging Personalization and Control in Scientific Personalized Search

Personalized search is a problem where models benefit from learning user preferences from per-user historical interaction data. The inferred preferences enable personalized ranking models to improve the relevance of documents for users. However, personalization is also seen as opaque in its use of historical interactions and is not amenable to users' control. Further, personalization limits the diversity of information users are exposed to. While search results may be automatically diversified this does little to address the lack of control over personalization. In response, we introduce a model for personalized search that enables users to control personalized rankings proactively. Our model, CtrlCE, is a novel cross-encoder model augmented with an editable memory built from users' historical interactions. The editable memory allows cross-encoders to be personalized efficiently and enables users to control personalized ranking. Next, because all queries do not require personalization, we introduce a calibrated mixing model which determines when personalization is necessary. This enables users to control personalization via their editable memory only when necessary. To thoroughly evaluate CtrlCE, we demonstrate its empirical performance in four domains of science, its ability to selectively request user control in a calibration evaluation of the mixing model, and the control provided by its editable memory in a user study.

==> figs/person-ablation-table.tex <==
\begin{table*}
\centering 
\caption{The various components of the \ctrlce ablated for both item (\ctrlceit) and concept-value (\ctrlcecv) memory to represent user documents.}
\scalebox{1}{
\begin{tabular}{lcccccccc}
\toprule
 & \multicolumn{2}{c}{Comp Sci} & \multicolumn{2}{c}{Physics} & \multicolumn{2}{c}{Pol Sci} & \multicolumn{2}{c}{Psych}\\ 
\cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}\cmidrule(lr){8-9}
Model & MRR & NDCG@10 & MRR & NDCG@10 & MRR & NDCG@10 & MRR & NDCG@10\\
\toprule
\ctrlceit & {0.6287} & {0.3223} & {0.6667} & {0.3657} & {0.6480} & {0.3378} & {0.6847} & {0.3704}\\
-- no $f_{\text{Mem}}$ & 0.5923 & 0.3010 & 0.6375 & 0.3440 & 0.6122 & 0.3164 & 0.6576 & 0.3465\\
-- no $f_{\text{CE}}$ & 0.4395 & 0.1994 & 0.4924 & 0.2424 & 0.4276 & 0.1997 & 0.5024 & 0.2450\\ 
-- no $g_{\text{Mix}}$ & 0.6144  & 0.3078 & 0.6458 & 0.3452 & 0.6329 & 0.3236 & 0.6642 & 0.3517\\
-- no calibration & 0.6100 & 0.3065 & 0.6699 & 0.3633 & 0.6344 & 0.3277 & 0.6759 & 0.3623\\
\midrule
\ctrlcecv & {0.6157} & {0.3118} & {0.6563} & {0.3583} & {0.6368} & {0.3310} & {0.6750} & {0.3614}\\
-- no $f_{\text{Mem}}$ & 0.5899 & 0.2936 & 0.6276 & 0.3344 & 0.6205 & 0.3151 & 0.6452 & 0.3368\\
-- no $f_{\text{CE}}$ & 0.3620 & 0.1675 & 0.4027 & 0.1981 & 0.3749 & 0.1792 & 0.4196 & 0.2060\\
-- no $g_{\text{Mix}}$ & 0.6085 & 0.3061 & 0.6367 & 0.3390 & 0.6327 & 0.3278 & 0.6516 & 0.3399\\
-- no calibration & 0.6141 & 0.3121 & 0.6580 & 0.3602 & 0.6384 & 0.3326 & 0.6772 & 0.3625\\
\bottomrule
%%%%%%%%
\end{tabular}
}
\label{tab-edps-person-ablation}
\end{table*}

==> figs/person-calibration-plots-it.tex <==
\begin{figure*}[t]
    \centering
    \subfloat[\centering \ctrlceit in Comp Sci]{{\includegraphics[width=4.3cm]{images/binned-calibvsnocalib-mixing_model_score_vs_crossencoder_metric-person_cs-itempersonce.png}}}%
    ~
    \subfloat[\centering \ctrlceit in Physics]{{\includegraphics[width=4.3cm]{images/binned-calibvsnocalib-mixing_model_score_vs_crossencoder_metric-person_physics-itempersonce.png}}}%
    ~
    \subfloat[\centering \ctrlceit in Pol Sci]{{\includegraphics[width=4.3cm]{images/binned-calibvsnocalib-mixing_model_score_vs_crossencoder_metric-person_political_science-itempersonce.png}}}%
    ~
    \subfloat[\centering \ctrlceit in Psych]{{\includegraphics[width=4.3cm]{images/binned-calibvsnocalib-mixing_model_score_vs_crossencoder_metric-person_psychology-itempersonce.png}}}%
    \caption{Scores produced by the mixing model $g_{\text{Mix}}$ used to combine $f_{\text{CE}}$ and $f_{\text{Mem}}$ as $f=w\cdot f_{\text{CE}} + (1-w)\cdot f_{\text{Mem}}$ plotted against the NDCG@10 metric for the rankings produced by $f_{\text{CE}}$. \ctrlceit (blue) is compared against the respective models trained without a calibrated objective (pink). Our calibrated objective ensures that $g_{\text{Mix}}$ remains proportional to $f_{\text{CE}}$ performance. Section \ref{sec-edps-calibeval} discusses these results further.}%
    \label{fig-edps-person-calibration-it}%
\end{figure*}
